$\delta^{(k)}$-Colouring of Cycle Related Graphs

With respect to a proper colouring of a graph $G$, we know that $\delta(G) \leq \chi(G) \leq \Delta(G)+1$. If distinct colours represent distinct technology types to be located at vertices the question arises on how to place at least one of each of $k$, $1\leq k < \chi(G)$ technology types together with the minimum adjacency between similar technology types. In an improper colouring an edge $uv$ such that $c(u)=c(v)$ is called a bad edge. In this paper, we introduce the notion of $\delta^{(k)}$-colouring which is a near proper colouring of $G$ with exactly $1\leq k < \chi(G)$ distinct colours which minimizes the number of bad edges.

==> structure.tex <==
%----------------------------------------------------------------------------------------
%Required Packages %
%----------------------------------------------------------------------------------------

\usepackage{amssymb,amsmath,amsthm,latexsym}
\usepackage{amsfonts}
\usepackage{graphicx,caption,subcaption}
\usepackage[pdftex,bookmarks,colorlinks=false]{hyperref}
\usepackage[hmargin=1.2in,vmargin=1.2in]{geometry}
\usepackage[mathscr]{euscript}
\DeclareMathOperator{\lcm}{lcm}

%----- Authors \& Affiliations --------------------------------
\usepackage[auth-lg,affil-sl]{authblk}
\setcounter{Maxaffil}{4}
%--------------------------------------------------------------

\allowdisplaybreaks

%----- Tikz Environments ---------------------------------------
\usepackage{float}
\usepackage{calc,tikz}
\usetikzlibrary{arrows,decorations.markings,positioning,shapes.geometric,}
\tikzstyle{vertex}=[circle, draw, inner sep=1pt, minimum size=4pt]
\newcommand{\vertex}{\node[vertex]}
\newcounter{Angle}

\tikzstyle{ann} = [fill=white,font=\footnotesize,inner sep=1pt]
\tikzstyle{arrow} = [thick,<-->,>=stealth]


%---------------- Tabule Envirionments -------------------------

\usepackage{multirow}
\usepackage{hhline}
\usepackage{booktabs}
\usepackage{longtable}

\usepackage{url}

%--------------------------------------------------------------------------------------------

%--------------------------------------------------------------------------------------------
%New Commands/Renew Commands %
%--------------------------------------------------------------------------------------------

\newcommand{\noi}{\noindent}
\newcommand{\N}{\mathbb{N}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\cP}{\mathscr{P}}
\newcommand{\J}{\mathscr{J}}
\newcommand{\s}{{\Large \varsigma}}

%---------------------------------------------------------------------------------------------
% New Theorem Environments%
%---------------------------------------------------------------------------------------------

\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{note}[theorem]{Note}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{conention}[theorem]{Convention}
\newtheorem{example}{Example}
\newtheorem{problem}{Problem}
\newtheorem{remark}{Remark}

%--------------------------------------------------------------------------------------------
% SPECIAL COMMANDS
%--------------------------------------------------------------------------------------------

\newcommand{\keywordsname}{Keywords}
\newenvironment{keywords}{
	\normalfont
	\list{}{
		\labelwidth0pt
		\leftmargin0pt \rightmargin\leftmargin
		\listparindent\parindent \itemindent0pt
		\parsep0pt
		\let\fullwidthdisplay\relax}
	\item[\hskip\labelsep\bfseries\keywordsname:] \small}{\endlist}

\newcommand{\mscname}{MSC 2010}
\newenvironment{msc}{
	\normalfont
	\list{}{
		\labelwidth0pt
		\leftmargin0pt \rightmargin\leftmargin
		\listparindent\parindent \itemindent0pt
		\parsep0pt
		\let\fullwidthdisplay\relax}
	\item[\hskip\labelsep\bfseries\mscname:] \small}{\endlist}

%-----------------------------------------------------------------------------------------
% Header and Footer%
%-----------------------------------------------------------------------------------------

\markboth {\hspace*{-9mm} \centerline{\footnotesize 
		$\delta^{(k)}$-Colouring of Cycle Related Graphs}
}
{ \centerline {\footnotesize 
		J. Kok and S. Naduvath. 
	}\hspace*{-9mm}}

%------------------------------------------------------------------------------------------

\allowdisplaybreaks

%------------------------------------------------------------------------------------------
